NAREOR: The Narrative Reordering Problem

Many implicit inferences exist in text depending on how it is structured that can critically impact the text's interpretation and meaning. One such structural aspect present in text with chronology is the order of its presentation. For narratives or stories, this is known as the narrative order. Reordering a narrative can impact the temporal, causal, event-based, and other inferences readers draw from it, which in turn can have strong effects both on its interpretation and interestingness. In this paper, we propose and investigate the task of Narrative Reordering (NAREOR) which involves rewriting a given story in a different narrative order while preserving its plot. We present a dataset, NAREORC, with human rewritings of stories within ROCStories in non-linear orders, and conduct a detailed analysis of it. Further, we propose novel task-specific training methods with suitable evaluation metrics. We perform experiments on NAREORC using state-of-the-art models such as BART and T5 and conduct extensive automatic and human evaluations. We demonstrate that although our models can perform decently, NAREOR is a challenging task with potential for further exploration. We also investigate two applications of NAREOR: generation of more interesting variations of stories and serving as adversarial sets for temporal/event-related tasks, besides discussing other prospective ones, such as for pedagogical setups related to language skills like essay writing and applications to medicine involving clinical narratives.

==> sections/IMPORTANT_TODOS_FOR_CAM-READY.tex <==
-Combine content into a single .tex file
-CUT DOWN TO 7 PAGES BODY!
-Go through AAAI cam-ready instructions and ensure no issues


DONE:

Add self-citations (survey, GenAug, NAREOR, ALOHA, SMERTI, SAPPHIRE, VisCTG, etc.) (only added a couple of these due to space and relevance)

Add link to GitHub repo

Fix references/links between sections and stuff in the rendered PDF

Maybe cite Bamman's paper for cam-ready? https://twitter.com/dbamman/status/1433862823214411776

IMPORTANT!!! DELETE THE NINESIZE OPTION ADDED TO AAAI22.STY FOR SMALLER FONT SIZE. and also change \ninesize to \small for all (or at least most) tables and captions.

==> sections/ethicsandimpact.tex <==
We collected NAREORC using AMT, in a manner consistent with terms of use of any sources and intellectual property and privacy rights of AMT crowd workers. Almost all source content for NAREORC was based on ROCStories \cite{mostafazadeh-etal-2016-generating}, an already publicly available and widely used dataset in NLP research.%Further, we ensured NAREORC's quality as poor annotations were discarded and the corresponding story was republished on AMT.\steven{include this last sentence or nah?} \varun{I think we should remove, this is more to do with our dataset quality for users not the ethics of process itself which is what 's needed here.}

Crowd workers were fairly compensated: \$1.5 per rewritten story, \$0.50 per fluency, coherence, and logic evaluation, \$0.50 per Plot-pres evaluation, and \$0.50 per interestingness evaluation, for roughly 5-7 min (the first) and 2 min tasks (latter three), respectively. This is at least 1.5-2 times the minimum wage in the U.S.A. of \$7.25 per hour (\$0.725 per 6 minutes and \$0.25 per 2 minutes).%\sy{I have scaled up interestingness from 0.17 dollars to 0.50 to be consistent with the others lol}

We neither solicit, record, request or predict any personal information pertaining to the AMT crowd workers, during the rewriting or evaluation studies.

We do not foresee any explicit way malicious actors could specifically misuse the data we collect, or models that could be trained on it, beyond the misuse that is possible in general with any transduction task or dataset (e.g summarization). Since our dataset could be used to learn a paraphrasing function, all possible misuses that are conceivable for other paraphrasing transforms (e.g. syntactic paraphrasing) are also conceivable using our dataset.%\sy{Need any changes here?}
